Implications of a Temperature Dependent IMF I: Photometric Template Fitting

A universal stellar initial mass function (IMF) should not be expected from theoretical models of star formation, but little conclusive observational evidence for a variable IMF has been uncovered. In this paper, a parameterization of the IMF is introduced into photometric template fitting of the COSMOS2015 catalog. The resulting best-fit templates suggest systematic variations in the IMF, with most galaxies exhibiting top-heavier stellar populations than in the Milky Way. At fixed redshift, only a small range of IMFs are found, with the typical IMF becoming progressively top-heavier with increasing redshift. Additionally, subpopulations of ULIRGs, quiescent- and star-forming galaxies are compared with predictions of stellar population feedback and show clear qualitative similarities to the evolution of dust temperatures.

==> mynotes.tex <==
%In practice, it is likely that the stars in a galaxy formed under a range of conditions, including different $T_{IMF}$.  In principle, there is no fundamental reason why temperature cannot be treated as an individual template property like stellar mass instead of a fit property like $z_{phot}$.  For this analysis, however, a single $T_{IMF}$ is fit for each galaxy, making it in some sense a luminosity-averaged $T_{IMF}$.  

%This is done for two reasons.  First, there is already a mathematical degeneracy between any change in the IMF and star formation history.  Typically a complex history would be required to mimic a different $T_{IMF}$ using a canonical Kroupa IMF.  However, this may not be true of more general linear combinations of different $T_{IMF}$, and photometric template fitting already suffers from significant degeneracies.  Second, on a more practical level, doing this properly would require significantly rewriting EAZY, whereas the goal here is to mimic existing techniques as closely as possible.  The resulting $T_{IMF}$ might be interpreted similarly to the single stellar population age coming from photometric template fitting.

%Each basis template also has an associated set of properties: stellar mass, metallicity, age, dust extinction and star formation rate. Given a linear combination of these templates corresponding to a galaxy, properties scaling with mass can be calculated using a light-weighted sum of the properties for the individual templates. Properties that do not scale with mass (metallicity and age) can be calculated the same way with an additional normalization. Essentially, for each galaxy, this entire template-fitting process gives a spectrum fit to photometry, a photmetric redshift, IMF temperature, and these five additional properties. These properties can then be compared to the values obtained from template fitting with a constant Milky Way IMF.
